Resource Allocation for Downlink Cellular OFDMA Systems: Part I - Optimal Allocation

In this pair of papers (Part I and Part II in this issue), we investigate the issue of power control and subcarrier assignment in a sectorized two-cell downlink OFDMA system impaired by multicell interference. As recommended for WiMAX, we assume that the first part of the available bandwidth is likely to be reused by different base stations (and is thus subject to multicell interference) and that the second part of the bandwidth is shared in an orthogonal way between the different base stations (and is thus protected from multicell interference). Although the problem of multicell resource allocation is nonconvex in this scenario, we provide in Part I the general form of the global solution. In particular, the optimal resource allocation turns out to be "binary" in the sense that, except for at most one pivot-user in each cell, any user receives data either in the reused bandwidth or in the protected bandwidth, but not in both. The determination of the optimal resource allocation essentially reduces to the determination of the latter pivot-position.

==> commandes.tex <==
% Packages


% Theoremes
\newtheorem{remark}{Remark}
\newtheorem{prop}{Proposition}
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{theo}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{conj}{Conjecture}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{corollary}{Corollary}


% Titres
\newcommand{\Headingtitre}[1]{\begin{center}\Large\bf\sc #1\end{center}}
\newcommand{\headingtitre}[1]{\begin{center}\large\bf\sc #1\end{center}}
\newcommand{\heading}[1]{\begin{center}\large \underline{#1}\end{center}}
\newcommand{\headingmf}[1]{\large\bf\it \underline{#1}}
\newcommand{\titre}[1]{\begin{center}\large\it {#1}\end{center}}


% Couleurs
\usepackage{color}
\definecolor{MyDarkBlue}{rgb}{0.1,0,0.65}
\definecolor{MyDarkRed}{rgb}{.85,0,0.1}

% Symboles 
\newcommand{\tr}[1]{\textrm{tr}\left(#1\right)}
\newcommand{\tri}{$\triangleright$}
\newcommand{\btri}{{\color{MyDarkBlue} $\triangleright$}}
\newcommand{\bbul}{{\color{MyDarkBlue} $\bullet$}}

% Espacement
\newcommand{\RR}{\vspace*{.2cm}\\}


% Macro math g\'en\'erales
\newcommand{\real}[1]{{\mathfrak{R}}\left[#1\right]}
\newcommand{\imag}[1]{{\mathfrak{I}}\left[#1\right]}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\diag}[1]{\textrm{diag}\left(#1\right)}
\newcommand{\trace}[1]{\textrm{Trace}\left(#1\right)}
\newcommand{\card}[1]{\textrm{card}\left(#1\right)}
\newcommand{\EE}[1]{{\mathbb{E}}\left[ #1 \right]}
\newcommand{\PP}[1]{{\mathbb{P}}\left\{ #1 \right\}}
\newcommand{\Pout}{{\mathbb{P}}_\textrm{out}}
\newcommand{\oo}{\textrm{o}}
\newcommand{\ud}{\textrm{d}}
\renewcommand{\i}{\imath}
%\renewcommand{\QED}{\QEDopen}
\providecommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\bs}{\boldsymbol}
\newcommand{\dsp}{\displaystyle}
\newcommand{\dron}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ddron}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\dddron}[3]{\frac{\partial^2 #1}{\partial #2 \:\partial #3}}

% Macro synchro
\newcommand{\df}{\delta\! f}
\newcommand{\dfk}{\delta\! f_k}
\newcommand{\ok}{\omega_k}
\newcommand{\CRBN}{\overline{CRB}_N}
\newcommand{\Nk}{_{N,k}}
\newcommand{\Nl}{_{N,l}}

% Macro relay
\newcommand{\Pc}{P_{\cal C}}
\newcommand{\Pco}{P_{{\cal C}_0}}
%\newcommand{\Tc}{{\cal T}_{\cal C}}
\newcommand{\Tco}{{\cal T}_{{\cal C}_0}}
\newcommand{\Sc}{{\cal S}_{\cal C}}
\newcommand{\Sco}{{\cal S}_{{\cal C}_0}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bXoo}{{\bf X}_{00}}
\newcommand{\bXou}{{\bf X}_{01}}
\newcommand{\bYuo}{{\bf Y}_{10}}
\newcommand{\bXuu}{{\bf X}_{11}}
\newcommand{\bYdo}{{\bf Y}_{20}}
\newcommand{\bYdu}{{\bf Y}_{21}}

% Macro Nassar
\newcommand{\ki}{_{k,i}}
\newcommand{\ku}{_{k,1}}
\newcommand{\kd}{_{k,2}}
\newcommand{\li}{_{l,i}}
\newcommand{\lu}{_{l,1}}
\newcommand{\ld}{_{l,2}}
\newcommand{\Lu}{_{L,1}}
\newcommand{\Lpu}{_{L+1,1}}
\newcommand{\Ld}{_{L,2}}
\newcommand{\Lpd}{_{L+1,2}}
\newcommand{\Lp}{_{L+1}}
\newcommand{\A}{{\cal A}}
\newcommand{\Au}{{\cal A}_1}
\newcommand{\Ad}{{\cal A}_2}
\newcommand{\Ai}{{\cal A}_i}
\newcommand{\K}{^{(K)}}
\newcommand{\cK}{^{c,(K)}}
\newcommand{\cpK}{^{c,(\phi_K)}}
\newcommand{\ctK}{^{c,(\theta_K)}}
\newcommand{\cpsiK}{^{c,(\psi_K)}}
\newcommand{\ApK}{^{A,(\phi_K)}}
\newcommand{\BpK}{^{B,(\phi_K)}}
\newcommand{\AK}{^{A,(K)}}
\newcommand{\BK}{^{B,(K)}}
\newcommand{\cbarK}{^{\overline{c},(K)}}
\newcommand{\QujA}{Q_{1,j}^A}
\newcommand{\QujB}{Q_{1,j}^B}
\newcommand{\QdjA}{Q_{2,j}^A}
\newcommand{\QdjB}{Q_{2,j}^B}
\newcommand{\QjA}{Q_{j}^A}
\newcommand{\QjB}{Q_{j}^B}
\newcommand{\QdiA}{Q_{2,\infty}^A}
\newcommand{\QdiB}{Q_{2,\infty}^B}
\newcommand{\QuiA}{Q_{1,\infty}^A}
\newcommand{\QuiB}{Q_{1,\infty}^B}
\newcommand{\QiA}{Q_{\infty}^A}
\newcommand{\QiB}{Q_{\infty}^B}
